Latent Association Mining in Binary Data

We consider the problem of identifying stable sets of mutually associated features in moderate or high-dimensional binary data. In this context we develop and investigate a method called Latent Association Mining for Binary Data (LAMB). The LAMB method is based on a simple threshold model in which the observed binary values represent a random thresholding of a latent continuous vector that may have a complex association structure. We consider a measure of latent association that quantifies association in the latent continuous vector without bias due to the random thresholding. The LAMB method uses an iterative testing based search procedure to identify stable sets of mutually associated features. We compare the LAMB method with several competing methods on artificial binary-valued datasets and two real count-valued datasets. The LAMB method detects meaningful associations in these datasets. In the case of the count-valued datasets, associations detected by the LAMB method are based only on information about whether the counts are zero or non-zero, and is competitive with methods that have access to the full count data.

==> tex/clt.tex <==
As discussed in Section \ref{sec:test}, the hypothesis testing in the
LAMB method's search procedure relies on empirical p-values
for estimates of the average latent association. %$\psi(i, A_{-i})$.
These p-values are derived from a central limit theorem that we now present in detail.
In what follows, let the $d$-dimensional random vectors $\bm{V}$, $\bm{\theta}$, and
$\bm{X} = \mathbbm{1}\left( \bm{V} \leq \bm{F}^{-1}(\bm{\theta}) \right)$
be as in Definition \ref{def:mod}.  For each $i \in [d]$ let
\begin{align}
	\label{eq:u}
	U_{i}  
		&:=  \frac{X_{i} - \theta_{i}}{ \sqrt{ \theta_{i} (1- \theta_{i}) } }
\end{align}
be the conditionally standardized $X_{i}$.  
For a subset $A \subseteq [d]$ denote
the average of $U_{i}$ over $i \in A$ by
\begin{align}
	\label{eq:v}
	U_{A}  
		&:=  \frac{1}{|A|} \sum_{i \in A} U_{i} \, ,
\end{align}
and define
\begin{align}
\label{eq:barpsi}
	\Psi(A)
		&:= \frac{1}{|A|^2} \sum_{i,k \in A} \psi(i,k)\,.
\end{align}
%be the average pairwise latent coherence between the variables in $A$.  
The next two lemmas establish some basic
properties of the quantities defined above in 
relation to latent association, i.e.,
Equations~\eqref{eq:lat_cor} and \eqref{eq:avg_coh}.
These lemmas are proved in Appendix~\ref{app:theory}.


\begin{lemma}
\label{lem:uv}
For each $i,k \in [d]$ and $A \subseteq [d]$:
%%\blue{such that $j\notin A$},
\begin{enumerate}

\item $\mathbb{E} (U_i) = 0$ and $\mathbb{E}( U_i^2) = 1$,

\item $\psi(i,k) = \mathbb{E} (U_i U_k)$ and $|\psi(i,k)| \leq 1$,

\item $\mathbb{E} (U_i U_A) = \psi(i,A)$ and $\mathbb{E}( U_A^2) = \Psi(A)$.

\item If $V_i$ is independent of $\{ V_k : k \in A \}$, then
	$\mathbb{E}(U_i U_A) = 0$ and 
	$\mathbb{E}( U_i^2 \, U_A^2) = \Psi(A)$. %= \mathbb{E} (U_A^2)$.
\end{enumerate}
\end{lemma}


\begin{lemma}
\label{lem:v4}
%Let $U_i$ and $U_A$ be defined as in \eqref{eq:u} and \eqref{eq:v}. Then
For each $i \in [d]$ and $A \subseteq [d]$:
\begin{enumerate}
\item $\mathbb{E} (U_i^4) \leq \min\left\{1, \mathbb{E} (\theta_i^{-1} (1 - \theta_i)^{-1})\right\}$
	and $\mathbb{E}(U_A^4 )
		\leq \min\left\{ 1, |A|^{-1} \sum_{k \in A} \mathbb{E}( \theta_k^{-1} (1 - \theta_k)^{-1})\right\}$.

\item If $V_i$ is independent of $\{ V_k : k \in A \}$, then \\
$\mathbb{E}(U_i^4 \, U_{A}^4) \leq 
	\min\left\{1,  |A|^{-1}  \sum_{k \in A} \mathbb{E} (\theta_i^{-1} (1 - \theta_i)^{-1} \theta_k^{-1} (1 - \theta_k)^{-1})\right\}$.
\end{enumerate}
\end{lemma}


With the above two lemmas, we now establish a central limit theorem 
for latent association in the following asymptotic setting.
For each $n \in\mathbb{N}$, let $\bm{V}_1, \ldots, \bm{V}_n \sim \mu_n$ and
$\bm{\theta}_1, \ldots, \bm{\theta}_n \sim \nu_n$ be independent random $d$-vectors. 
Note that the distributions $\mu_n$ and $\nu_n$ %, as well as the dimension $d_n$, \red{WHY can $d$ depend on $n$?!}
may depend on $n$.
For each $n\in\mathbb{N}$ and $j \in [n]$, let $\bm{X}_{\cdot j} = \mathbbm{1}\{ \bm{V}_j \leq \bm{F}_n^{-1}(\bm{\theta}_j )\}$ 
be the binary-valued random vectors generated under the threshold model of Definition~\ref{def:mod},
where $\bm{X}_{\cdot j} := (X_{1j}, \ldots, X_{dj})^t$.

Let $\widehat{\psi}_n(i, k)$ be the sample latent association 
between features $i$ and $k$,
defined in \eqref{eq:sam_coh}, and let
$U_{Aj}$ be defined as in  \eqref{eq:v} for each $j\in [n]$.  
Then a natural estimate of $\psi(i,A) = \Ex (U_i \, U_A)$ is the sample average
\begin{align}
\label{eq:psihat}
	\widehat{\psi}_n (i, A)
		&:= \frac{1}{|A|} \sum_{k\in A} \widehat{\psi}_n(i,k)
			\overset{\text{\eqref{eq:sam_coh}}}{=} \frac{1}{n} \sum_{j \in [n] } U_{ij} \, U_{Aj}\,.
\end{align}
It follows from Lemma~\ref{lem:uv} that $\Ex [\widehat{\psi}_n (i, A) ]= \psi(i, A)$.  Furthermore,
if $V_i$ is independent of $\{ V_k : k \in A \}$, then 
%%$\Ex \widehat{\psi}_n (j, A) = \psi(j,A) = \Ex (U_{1j} \, U_{1A}) = 0$ 
%$\Ex [\widehat{\psi}_n (i, A)] = 0$ and 
the independence over $j\in [n]$ together implies that
\begin{align*}
	\text{Var}\left(\sqrt{n} \, \widehat{\psi}_n (i, A) \right) 
		&= \frac{1}{n} \sum_{j\in [n]}\text{Var}( U_{ij} U_{Aj}) 
			= \mathbb{E} ( U_{i1}^2  U_{A1}^2 ) = \Psi(A) .
\end{align*}
In particular, %when $V_i$ is independent of $\{V_k\in k\in {A}\}$ we have
%%\beq
%%\label{eq:sample_var}
%%\hat{\sigma}^2_n (i, A)  := \frac{1}{n} \sum_{j \in [n]}  U_{ij}^2 U_{Aj}^2 
%%\eeq
\begin{align}
	\widehat{\sigma}^2_n (i, A)  
		&:= \frac{1}{n}\sum_{j\in [n]} U_{Aj}^2 \label{eq:sample_var}
\end{align}
is an unbiased estimator of the variance of $\sqrt{n} \, \widehat{\psi}_n (i, A)$.
We note that another unbiased estimator of the variance of $\sqrt{n}\,\widehat{\psi}_n(i, A)$ 
is $\widehat{s}^2_n(i, A) := \frac{1}{n}\sum_{j\in [n]} U^2_{ij}U^2_{Aj}$,
whenever $V_i$ is independent of $\{V_k\colon k\in {A}\}$. 
Both of these variance estimates are unbiased estimators of $\Psi(A)$,
and both converge in probability to $\Psi(A)$, under the same assumptions
used below.
However, $\widehat{\sigma}^2_n(i, A)$ is computationally 
more efficient than $\widehat{s}^2_n(i, A)$. 
This is because $\widehat{\sigma}^2_n(i, A)$ can be calculated and stored outside of 
the iterative testing algorithm,
discussed in Section~\ref{sec:lamb}. The key difference is the lack of dependence on $i$ in 
$\widehat{\sigma}^2_n(i, A)$, which makes calculations more efficient
across updates to $A$ during the iterative testing algorithm. 


We are now ready to state the central limit theorem for latent association.
This establishes the empirical p-values used in the iterative testing procedure, 
as described in Sections~\ref{sec:lamb} and~\ref{sec:test}.
The proof follows from two lemmas 
that are proved in Appendix~\ref{app:theory}.

\begin{theorem}{\bf(Central Limit Theorem for Sample Latent Association)}
\label{thm:csm_clt}
Fix $i \in [d]$ and for each $n\in \mathbb{N}$ let $A_n \subset [d]\backslash \{i\}$ be an index set with cardinality $m_n :=|A_n|$.
Let $\widehat{\psi}_n (i, A_n)$ be the sample latent association of $i$ and $A_n$ under $(\mu_n, \nu_n)$
and let $\widehat{\sigma}^2_n (i, A_n)$ be defined as in (\ref{eq:sample_var}).
Assume that
\begin{enumerate}
	\item for each $n$, $V_i$ is independent of $\{ V_k : k \in A_n \}$ under $\mu_n$;
	\item \begin{align*} 
		\Psi(A_n)^{-2} \left( {1 \over m_n} \sum_{k \in A_n} \Ex \left[\theta_i^{-1}(1-\theta_i)^{-1} \theta_k^{-1}(1-\theta_k)^{-1}  \right] \right)
	  		&= o(n) \, .
		\end{align*}
\end{enumerate}
Then,
\begin{align}
\label{eq:clt2}
 	\frac{\sqrt{n}\, \widehat{\psi}_n (i, A_n)} {\widehat{\sigma}_n(i, A_n)}
		&\overset{d}{\to}  \mathcal{N}(0,1) \quad\textnormal{as  $n \to \infty$} .
\end{align}
\end{theorem}



\noindent
\emph{Proof.}
The theorem is a corollary of Slutsky's theorem and Lemmas~\ref{lem:csm_clt}
and \ref{lem:sigma}.
\qed



\begin{lemma}
\label{lem:csm_clt}
Under the conditions of Theorem~\ref{thm:csm_clt},
\begin{align}
	\label{eq:clt}
	\frac{\sqrt{n} \, \widehat{\psi}_n (i, A_n)} {\Psi(A_n)^{1/2}}
		&\overset{d}{\to} \mathcal{N}(0,1) \quad\textnormal{as  $n \to \infty$.}
\end{align}
\end{lemma}




\begin{lemma}
\label{lem:sigma}
Under the conditions of Theorem \ref{thm:csm_clt},
\begin{align}
	\label{eq:var_consis}
		\left| \frac{\widehat{\sigma}_n^2(i, A_n) }{\Psi(A_n)} - 1 \right| \overset{p}{\to} 0 \quad\textnormal{as $n\to \infty$}.
\end{align}
\end{lemma}


==> tex/est_thresholds.tex <==
The hypothesis testing approach outlined in 
Sections~\ref{sec:test} and \ref{sec: CLT}
requires that $\mathbf{\Theta}_{d \times n} = [\bm{\theta}_{\cdot 1}, \ldots, \bm{\theta}_{\cdot n}]$ 
be known alongside the observed $\mathbb{X}_{d \times n} = [x_{ij}]
\in \{0, 1\}^{d \times n}$. %= [\bm{X}_{\cdot 1}, \ldots, \bm{X}_{\cdot n}]$.  
However, in our generative model
$\bm{\theta}_{\cdot 1}, \ldots, \bm{\theta}_{\cdot n}$ are not  observable, 
they are latent random vectors. 
Our approach is to derive consistent estimators of %$\mathbf{\Theta}$ 
$\bm{\theta}_{\cdot 1}, \ldots, \bm{\theta}_{\cdot n}$
from the data matrix $\mathbb{X}$.  
The details of this estimation procedure is discussed
in this section.
We then treat these estimates as observed values and plug them 
directly into the sample latent association defined in Section~\ref{sec: CLT}
Equation \eqref{eq:sam_coh}.  
Results from simulated and real data applications, 
as well as the asymptotic consistency of our estimators, 
suggests that this is a reasonable approximation.

In Section~\ref{subsec: theta model} we discussed
the Truncated Poisson Factorization Model (TPFM)
for the random thresholds $\bm{\theta}_{\cdot 1}, \ldots, \bm{\theta}_{\cdot n}$.
%The TPFM reduces the effective dimension of $\mathbf{\Theta}$,
%allowing us to efficiently estimate $\mathbf{\Theta}$ from $\mathbb{X}$.  
Under the TPFM %parameter model of Definition~\ref{def: threshold model}
%in Section~\ref{subsec: theta model}, 
the random thresholds $\bm{\theta}_{\cdot 1}, \ldots, \bm{\theta}_{\cdot n}$ 
depend on a random sample $\tau_1, \ldots, \tau_n$  from $\pi$
and deterministic parameters $\alpha_1, \cdots, \alpha_d$. 
Therefore the number of quantities to estimate is reduced from 
$d \cdot n$ realized values of $\{ \theta_{ij} \}$ to $d + n$ parameters 
$(\alpha_1, \ldots, \alpha_d, \tau_1^0, \ldots, \tau^0_n)$,
where $\tau_j^0$ is a realized value of $\tau_j\sim \pi$. %, 
%which fully specify $\mathbf{\Theta}$
%for our purposes of conditioning.  
In this sense, we can think of the TPFM as a sort of 
``rank-one'' approximation of %the distribution $\nu$  %for observation ``preferences''.
$\mathbf{\Theta}$.
Under certain mild conditions, described below,
we can efficiently estimate $\mathbf{\Theta}$ from $\mathbb{X}$. %,
%which we consider in Section~\ref{subsec: parameter consistency}. %\ref{sec:params}. 
%%In particular, since in many practical cases \blue{most} $\theta_{ij}$'s are small, 
%%we focus on the case when their expected values tend towards 0.

%As discussed earlier, for a given $j\in [n]$ and all $i\in [d]$,
%the TPFM defines $\theta_{ij}$ marginally as a function of 
%a positive-valued random variable $\tau_j$
%and a fixed positive-valued rate parameter $\alpha_i$.
%The parameter $\tau_j$ captures  a notion of resource or budget
%for sample $j$, while the parameter 
%$\alpha_i$ captures an intrinsic popularity or utility  of feature $i$
%for all samples in the population.
%This assumption for the random thresholds helps us model 
%heterogeneity in samples. %, i.e.,
%drop the assumption of identically distributed samples.
%%In other words, we assume that the dependence structure and 
%%randomness of $\bm{\theta}_{\cdot j}$ derives from a single shared random variable $\tau_j$.  
%%Differences between the marginal distributions of $\theta_{1j}, \ldots, \theta_{dj}$ 
%%are then entirely captured by the fixed parameters $\bm{\alpha} = (\alpha_1, \ldots, \alpha_d)$.






\subsection{Estimation Consistency}
\label{subsec: parameter consistency}

Throughout this section we consider the asymptotic 
setting as in Section \ref{sec: CLT} for Definition \ref{def:mod} 
and Equation \eqref{eq:theta}, where $\bm{\theta} \sim \nu_n$.
First we consider the consistency in estimating the expected value of $\bm{\theta} \sim \nu_n$.
Note that $\mathbb{E}(X_{i}) = \mathbb{E}(\mathbb{E}[X_{i}|\bm{\theta}])
=\mathbb{E}(\theta_{i})$. Therefore, unconditionally for each $i\in[d]$, 
$X_{i1}, \ldots, X_{in} \overset{\textnormal{iid}}{\sim} \textnormal{Bernoulli}(\mathbb{E}(\theta_{i}))$,
and a natural estimate of $\mathbb{E}(\theta_{i})$ is  $ \overline{X}_{i} := \frac{1}{n} \sum_{j=1}^n X_{ij}$. 
We have the following theorem on the consistency of $\overline{X}_{i}$ when 
$\{\mathbb{E}(\theta_{i})\}_{i\in[d]}$ are small, but not too small.
For example, when $\{\mathbb{E}(\theta_{i})\}_{i\in[d]}$ are uniformly bounded from below.

\begin{prop}
\label{prop:theta_mean}
Suppose we have the following condition on $\{\mathbb{E}(\theta_{i})\}_{i\in[d]}$:
\begin{align*}
	\varlimsup_{n \rightarrow \infty} \frac{1}{n} \max_{i \in [d]} \frac{1}{\mathbb{E}(\theta_i)}
		&= 0.
\end{align*} 
Then we have the following convergence:
 \begin{align*}
  	\max_{i\in [d]} \left| \frac{\overline{X}_{i} }{ \mathbb{E}(\theta_i) } - 1 \right|  \stackrel{p}{\longrightarrow} 0
		\quad\textnormal{as $n\to\infty$}.
\end{align*}
\end{prop}

\noindent
\emph{Proof.}
Fix arbitrary $n\in\mathbb{N}$ and $\epsilon > 0$.
By Chebyshev's inequality and the condition on $\{\mathbb{E}(\theta_{i})\}_{i\in[d]}$, %for any %\blue{$j\in [d_n]$} and any 
\begin{align*}
	\max_{ i \in [d]} \mathbb{P}\left(\left| \frac{\overline{X}_{i} }{ \mathbb{E}(\theta_i) } - 1 \right|  > \epsilon \right) 
		&\leq \frac{1}{n \epsilon^2} \max_{ i \in [d]}  \left[\frac{1}{\mathbb{E}(\theta_i)} -1\right]= o(1).
\end{align*}
\qed

An immediate consequence of Proposition~\ref{prop:theta_mean} 
is the estimation of $\alpha_{i}$
for  $i\in [d]$. From Equation~\eqref{eq:theta} we see that 
\begin{align*}
	\mathbb{E}(\theta_i) 
		&= h(\alpha_{i})  :=   \int_\mathcal{T} \left( 1 - e^{- t \alpha_{i}} \right)  \pi(t) \,\textnormal{d}t,
\end{align*} 
where $\mathcal{T}$ is the support of $\tau\sim \pi$.
Suppose that the condition on $\{\mathbb{E}(\theta_{i})\}_{i\in[d]}$ 
in Proposition~\ref{prop:theta_mean} is satisfied.
If the distribution of $\tau \sim \pi$ leads to a function $h$ that is %continuous and 
invertible with $\mathbb{E}(\theta_i)\in C_{h^{-1}}:= \{x: h^{-1} \textnormal{ is continuous at } x\}$, 
then the Continuous Mapping Theorem implies that 
$h^{-1} (\overline{X}_{i})$ is consistent for $\alpha_i$. %$h^{-1} (\mathbb{E}(\theta_i))=\alpha_{i}$


To completely estimate $\mathbf{\Theta}$ we must also estimate 
the unobserved realized values of the random variables 
$\tau_1, \ldots, \tau_n$.
We denote by $\tau_1^0, \ldots, \tau_n^0$ these realized values.  
Consider the posterior distribution of 
$\tau\sim \pi$ given $\bm{X}_{\cdot j} = \bm{x}_{\cdot j}:=(x_{1j}, \ldots, x_{dj})^T$ 
and $\bm{\alpha}_n := (\alpha_1^n,\ldots, \alpha_{d}^n)^t$, 
which we denote by $\pi(\cdot \given \bm{X}_{\cdot j}, \bm{\alpha}_n)$.  
A straightforward estimator for $\tau_j^0$ is the posterior mean
\begin{align}
	\mathbb{E}[ \tau_j \given \bm{X}_{\cdot j}, \bm{\alpha}_n ]
		&=  \int_0^{\infty}  t \,\pi(t \given \bm{X}_{\cdot j}, \bm{\alpha}_n) \, \textnormal{d}t  \, .
\end{align}
The following result guarantees consistency of the posterior mean.  We appeal directly to Theorem 4.1 of \citet{suman}, which requires the following condition on the prior $\pi$ for $\tau$.


\begin{condition}   
\label{cond: tau prior}
For each $\delta>0$ there exist sets $\{S_k\}_{k\in\mathbb{N}}$ 
such that the diameter of each set is less than 
$\delta$, $\cup_{k \in \mathbb{N}} S_k = \mathbb{R}^{+}$, 
and $\sum_{k \in\mathbb{N}}{\sqrt{\pi(S_k)}} < \infty$.
\end{condition}

\begin{remark} 
In essence, Condition~\ref{cond: tau prior} is a 
concentration condition for $\pi$, guaranteeing 
that the measure is not too spread out over the support of $\tau$.
\end{remark}

\begin{theorem}{\bf (\citet{suman})}
\label{thm:taus}
    Suppose that Condition~\ref{cond: tau prior} holds and that  
    $\mathrm{\pi}(\cdot \given \bm{X}_{\cdot j}, \bm{\alpha}_n)$ is bounded. Then, for every $\epsilon > 0$,
    \begin{align*}
    	\mathbb{P}\left( \left| \mathbb{E}[ \tau_j \given \bm{X}_{\cdot j}, \bm{\alpha}_n ] - \tau_j^0 \right| > \epsilon \right) \to 0
    \end{align*}
    as $n \to \infty$. The probability is taken over 
    the distribution of $(\bm{X}_n, \bm{\theta}_n)$ derived
    from the product measure $(\mu_n, \nu_n)$.
\end{theorem}

In practice $\bm{\alpha}_n$ is not known, so we instead estimate 
$\tau_j^0$ by plugging in consistent estimates 
$(\widehat{\alpha}^n_{1}, \ldots, \widehat{\alpha}^n_{d} )$, i.e.,
\begin{align}
	\label{eq:tau}
	\widehat{\tau}_j^n
		&:= \mathbb{E}[ \tau_j \given \bm{X}_{\cdot j}, \widehat{\bm{\alpha}}_n ]
			=  \int_0^{\infty}  t \pi(t \given \bm{X}_{\cdot j}, \widehat{\bm{\alpha}}_n)\, \textnormal{d}t  \, .
\end{align}
Then, for all $n\in\mathbb{N}$, $j \in [n]$, and $i \in [d]$, 
$\theta_{ij}$ is estimated 
by $\widehat{\theta}_{ij}(n) := 1-e^{-\widehat{\alpha}_{i} ^n\widehat{\tau}_j^n }$.

The following proposition provides a general family 
of models which satisfy the conditions in 
Theorem~\ref{thm:csm_clt} and Proposition~\ref{prop:theta_mean}.
\begin{prop}
\label{prop:prior}
Consider the Gamma($\zeta$, $\beta$) as the prior distribution 
$\pi$ for $\tau$, with density
\begin{align*}
	f_\tau(x) 
		&= \frac{\beta^\zeta}{\Gamma(\beta)} x^{\zeta -1} \exp{\left(-\beta x\right)}.
\end{align*}
As in Theorem~\ref{thm:csm_clt},
fix $i \in [d]$ and for each $n\in \mathbb{N}$ let $A_n \subset [d]\backslash \{i\}$ 
be an index set with cardinality $m_n := |A_n|$. Assume the following:
\begin{enumerate}
  \item $\min_{i \in [d]} n\alpha_i \rightarrow \infty$.
  \item $\max_{i \in [d]} \alpha_i \leq M\in (0, \infty)$.
  \item Let $c_n := \min_{i \in [d]}\alpha_i$ 
  	and $\rho_n := \lambda_{\min} \left(\Sigma(A_n)\right)$,
	the minimal eigenvalue of the matrix
	$\Sigma(A_n) := [\psi(l,k)]_{l,k \in A_n}$. 
	Then $\frac{m_n}{n c_n^2 \rho_n^{2}}\rightarrow 0$.
\end{enumerate}
Then the Gamma($\zeta$, $\beta$) prior with $\beta>6M$ and $\zeta \geq3$ satisfies:
\begin{enumerate}
  \item $\Psi(A_n)^{-2}\left(\frac{1}{m_n} \sum_{k \in A_n}\mathbb{E}\left[\theta_i^{-1}  (1-\theta_i)^{-1} \theta_k^{-1}(1-\theta_k)^{-1}\right] \right) =o(n)$ 
  		as in Theorem~\ref{thm:csm_clt}.
  \item $\varlimsup_{n \rightarrow \infty}\frac{1}{n} \max_{i \in [d]} \frac{1}{\mathbb{E}(\theta_i)} =0$ 
  		as in Proposition~\ref{prop:theta_mean}.
\end{enumerate}
\end{prop}

\begin{remark}  
The three assumptions in Proposition~\ref{prop:prior} are mild for practical use. 
For example, if $\rho_n =O(1)$, $c_n>>\frac{1}{n^{1/4}}$ then the assumptions
hold when $m_n << {n^{1/2}}$.
\end{remark}

\subsection{Implementation}
\label{sec:tildes}


The consistent estimators derived in Proposition \ref{prop:theta_mean} and 
Theorem \ref{thm:taus} rely on the distribution $\pi$ %, 
%and thus the function $h$, 
being known.  In practice, we generally do not know 
nor wish to assume the distribution of $\tau$.
A major consequence of our lack of assumptions 
for the underlying distributions of $\bm{V}$ and $\pi$
is that we do not know the joint distribution for the threshold model
of Definition~\ref{def:mod}. This prevents us 
from using standard EM or Variational Inference algorithms.
Our approach is to approximate the consistent 
estimators via an empirical distribution function.  
We replace the unknown prior $\pi$ with an empirical distribution function
\begin{align*}
%	\label{eq:prior}
	\hat{\pi}_n (t)
		&= \begin{cases}
			\frac{1}{n}, &\text{if} \tab t \in \{ \tau_1^0, \ldots, \tau_n^0 \} \\
			0, & \textnormal{otherwise.}
		\end{cases}
\end{align*}
Then the estimation approach suggested by Proposition \ref{prop:theta_mean} and 
Theorem \ref{thm:taus} is to maximize an approximation to the posterior likelihood for $\tau$ 
under an appropriate ``moment-of-moments'' estimation of $\bm{\alpha}$.  

To approximate the unknown joint likelihood for each $j\in[n]$ we use
\begin{align}
	\label{eq: tau pseudolikelihood}
	f(\bm{X}_{\cdot j}|\bm{\alpha}, \tau^0_j)
		&\approx \prod_{i = 1}^d  \left(1 - e^{ - \alpha_i \tau^0_j }\right)^{X_{ij}} \left(e^{- \alpha_i \tau^0_j }\right)^{(1- X_{ij})}\,.
\end{align}
%i.e., a factorized form across the variables that share $\tau_j^0$.
This is sometimes called a Pseudo-likelihood approach. (CITE relevant papers)
\red{Actually, this is more like the naive conditional independence assumption
used in Naive Bayes classification.}
The ``moment-of-moments'' estimation problem is
\begin{align}
	\label{eq: alpha MoM}
	\overline{X}_i
		&:= \frac{1}{n} \sum_{j\in [n]} X_{ij} 
			\approx \frac{1}{n} \sum_{j\in [n]} (1 - e^{- \alpha_i \tau_j^0}).
\end{align}
Equation~\eqref{eq: alpha MoM} is based on the result that
$\mathbb{E}(X_{ij}) = \mathbb{E}(\theta_{ij})$ for each $i\in [d]$ and $j\in [n]$
under our model assumptions.

Using the approximation to the joint likelihood
given by Equation~\ref{eq: tau pseudolikelihood}, we 
want to minimize the negative logarithm with respect to the $\tau$ 
parameters. Using a smoothed version of the ``moment-of-moments'' 
Equation~\ref{eq: alpha MoM},
we minimize with respect to the $\alpha$ parameters.
It is possible to do this latter optimization for 
estimating $\bm{\alpha}$ subject to a constraint that ensures convexity.
However, in practice we found that
the feasible convex set of this constraint does not 
seem to be large enough for robust estimation of the random thresholds.
See Appendix~\ref{app: conv opt theory} for details about the 
constraint that gives a convex optimization problem.

The optimization problems can be expressed as equations by
\begin{align}
	\hat{\tau}_i^0 | \bm{\alpha}
		&:= \argmin_{t\in (0,\infty)} \sum_{j\in [d]} \left[\alpha_j t - X_{ij}\left( \alpha_j t + \ln[1 - \exp(-\alpha_j t) ]\right) \right]
		\label{eq: opt eq ell}\\
	\hat{\alpha}_j | \bm{\tau}^0
		&:= \argmin_{a\in (0,\infty)} \left(\overline{X}_j - \frac{1}{n} \sum_{i\in [n]} \left[1 - \exp(- a \tau_i^0) \right] \right)^2
		\label{eq: opt eq mom}\\
		&\textnormal{subject to} \quad \frac{1}{n}\sum_{i\in [n]} \exp(-a \tau_i^0)
			\geq 1 - \overline{X}_j - s(a, \bm{\tau}^0) 
			\label{eq: opt eq convexity}\\
			&\textnormal{where} \quad s(a, \bm{t}) := \frac{\left[\frac{1}{n} \sum_{i\in[n]} t_i e^{-a t_i} \right]^2}{\frac{1}{n} \sum_{i\in [n]} t_i^2 e^{-a t_i}}. \label{eq: opt eq slack var}
\end{align}
Although these equations have no closed form solution, they can be computed 
to within arbitrary error by an ordinary MM algorithm (see, for example, \citet{MM}). 
\red{[not convinced we employ an MM algorithm though]} 
\blue{Maybe we don't have to comment on this?}
Proposition~\ref{prop:theta_mean} and Theorem~\ref{thm:taus} 
provide reassurance of the theoretical validity of these %estimators, 
optimization problems,
since they are an empirical approach to the consistent estimation 
of $\tau_1^0, \ldots, \tau_n^0$ and $\alpha_1, \ldots, \alpha_d$.
%in Proposition \ref{prop:theta_mean} and Theorem \ref{thm:taus}.
Despite the theoretical advantages of the estimators using a known prior $\pi$, 
we find that the empirical approach is more robust in real data settings. %, 
%since $\pi$ is commonly unknown.

%With the empirical prior \eqref{eq:prior}, we arrive at the following optimization problem:

%%\subsubsection{Old Version}
%%
%%\begin{align}
%%	 \label{eq:solve}
%%	\hat{\tau}_i &:= 
%%	\argmaxx_{\tau_i \in \blue{(0,\infty)} } \; \; \prod_{j = 1}^\blue{d}  \left(1 - e^{ - \alpha_j \tau_i }\right)^{X_{ij}} \left(e^{ - \alpha_j \tau_i }\right)^{(1- X_{ij})}\quad\blue{\textnormal{for each $i\in[n]$},} \\[.1in]
%%%	&\text{subject to} \tab
%%	\hat{\alpha}_j
%%		&:= \argmin_{\alpha_j\in (0,\infty)}
%%			\left| \overline{X}_{j} - \frac{1}{n} \sum_{i = 1}^n \left(1 - e^{ - \alpha_j \tau_i } \right) \right|
%%			\quad\blue{\textnormal{for each $j\in [d]$.}}\hspace{1in}
%%\end{align}

%%\noindent \blue{
%%[Note that I am not yet confident in this optimization procedure, 
%%because I think this likelihood is incorrect. Will talk to Kai about it,
%%Andrew thinks it is an appropriate approximation since $\tau_i$
%%is shared across the variables.
%%I feel like this subsection has the most room for improvement.]
%%[Based off 7/24 meeting with Kai, we should double check this 
%%likelihood optimization and consider
%%using a prior on pi instead, especially since we 
%%have some theoretical results for gamma prior.]
%%}



%%\blue{[Probably can scrap this entire paragraph, will save it for now.]}
%%In the \blue{LAMB} software, we also supply an option to compute $\widehat{\tau}_1, \ldots,  \widehat{\tau}_n$ and $\widehat{\bm{\alpha}}_n$ under an assumed gamma prior, as in Proposition~\ref{prop:prior}.  This option should only be used when there is a compelling reason to believe the prior $\pi$ is known to be gamma with a particular rate and shape.  





==> tex/intro.tex <==
A common problem in data analysis is identifying relational 
structure between features based on a sample.
The class of methods that address this problem 
%may be broadly 
is often called association mining.
In this paper we introduce a new statistical 
method for association mining of binary data, 
Latent Association Mining in Binary Data (LAMB). %,
%that attempts to address these issues.

The LAMB method is  built  on three components.
The first component is a simple threshold model.
In this model, binary observations are obtained by 
random thresholding of a continuous random vector. 
The continuous random vector and the random
threshold vector are independent and neither are 
observed in this model.
A truncated random Poisson factorization distribution captures the 
behavior of the random thresholds.  
Such a threshold model is of limited complexity, but is flexible
enough to capture heterogeneity among samples and features in datasets.
The second component in the LAMB method is
an association statistic, called latent association, that arises naturally from the 
threshold model.
The third component is the use of an iterative hypothesis testing 
search procedure to identify sets of features that
are positively associated. 


Like most existing association mining
methods, the search procedure that
we employ effectively searches the lattice of sets 
of features to detect association. The 
search procedure that we use in the LAMB
method is computationally efficient, so it can be applied 
to high-dimensional datasets.
In contrast to many conventional methods,
the LAMB method is carried out in a 
statistical framework and based on 
meaningful hypothesis tests. This
allows the LAMB method to
account for sample heterogeneity
and moderate false discoveries in both
real and artificial datasets discussed in this paper.



In Section~\ref{subsec: motivating example} we give
some motivation for a model of binary data with
sample heterogeneity.
In particular, the motivating example explains
the usefulness of latent association.
%Then in Section~\ref{subsec: notation} we briefly
%describe applications of the LAMB
%method to real datasets. Finally, i
In Section~\ref{subsec: organization}
we go through the organization of the rest of the paper.


\subsection{Motivating Example}
\label{subsec: motivating example}

We consider market basket data
to motivate the LAMB method.
Conventional association mining methods were 
originally applied to 
binary-valued market basket data.\footnote{Binary-valued 
data was due to both barcode and data storage 
technology at the time. The datasets 
did not necessarily reflect purchases made all at once.
(CITE AGARWAL and 2006 association mining survey)}
In market basket data 
the observations are individual buyer transactions
and the features are the items available for purchase.
These datasets typically contain sample heterogeneity. 
One buyer's decision to purchase a particular item 
can depend on two different criteria.
The first criteria is the buyer's valuation of that item
relative to other items.
The second criteria is the buyer's relative needs, 
financial budget, available time at the store, etc.
When applied to market basket data, 
the LAMB method tries to identify intrinsically associated 
sets of items while simultaneously accounting for 
such buyer heterogeneity.


Figure~\ref{tab: toy dataset} represents a toy market basket
dataset with 12 buyers and 14 items.
The $(i,j)$ entry of the table indicates
whether or not item $i$ was purchased by buyer $j$.
A 1 means that buyer $j$ purchased item $i$,
and a 0 means that buyer $j$ did not purchase item $i$.
Note the heterogeneity among observations:
observations 1--5 are high-volume buyers;
observations 6 and 7 are intermediate-volume buyers; 
and observations 8--12 are low-volume buyers.
From analyzing this toy dataset, as well as the analysis of real and 
artificial datasets discussed in Sections~\ref{sec: applications} and \ref{sec: sim study}, 
we demonstrate how our method differentiates itself from existing methods.


\begin{figure}
\centering
\small
Buyers\\
\vspace{.2cm}
\begin{tabular}{ccccccccccccc}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12\\
  \hline
 Item 1 &   0 &   0 &   0 &   0 &   0 &   1 &   0 &   1 &   1 &   1 &   1 &   1 \\
  Item  2 &   0 &   0 &   0 &   0 &   0 &   0 &   1 &   1 &   1 &   1 &   1 &   1 \\
  Item  3 &   1 &   1 &   1 &   1 &   1 &   1 &   0 &   0 &   0 &   0 &   0 &   0 \\
  Item  4 &   1 &   1 &   1 &   1 &   1 &   0 &   1 &   0 &   0 &   0 &   0 &   0 \\
  Item  5 &   1 &   1 &   1 &   1 &   0 &   1 &   0 &   0 &   0 &   0 &   0 &   0 \\
  Item  6 &   1 &   1 &   1 &   0 &   1 &   0 &   1 &   0 &   0 &   0 &   0 &   0 \\
 Item   7 &   1 &   1 &   0 &   1 &   1 &   1 &   0 &   0 &   0 &   0 &   0 &   0 \\
 Item   8 &   1 &   0 &   1 &   1 &   1 &   0 &   1 &   0 &   0 &   0 &   0 &   0 \\
  Item  9 &   0 &   1 &   1 &   1 &   1 &   1 &   0 &   0 &   0 &   0 &   0 &   0 \\
  Item  10 &   1 &   1 &   1 &   1 &   1 &   0 &   1 &   0 &   0 &   0 &   0 &   1 \\
  Item  11 &   1 &   1 &   1 &   1 &   1 &   1 &   0 &   0 &   0 &   0 &   1 &   0 \\
  Item  12 &   1 &   1 &   1 &   1 &   1 &   0 &   1 &   0 &   0 &   1 &   0 &   0 \\
   Item 13 &   1 &   1 &   1 &   1 &   1 &   1 &   0 &   0 &   1 &   0 &   0 &   0 \\
   Item 14 &   1 &   1 &   1 &   1 &   1 &   0 &   1 &   1 &   0 &   0 &   0 &   0 \\
   \hline
\end{tabular}
\caption{Toy market basket dataset.}
\label{tab: toy dataset}
\end{figure}

A commonly used statistical measure of association is Pearson correlation.
However, using correlation when sample heterogeneity is present
in a dataset may lead to spurious results.
Consider the item sets \{1, 2\} and \{3, 4\}.  
These two sets show identical behavior up to a permutation of the observations.  
In particular, the correlation between the two items in each set
is the same ($r_{12} = r_{34} = 0.667$). The two items
in each set are also equally far apart in both 
$\ell_1$ and $\ell_2$ distance ($d_{12}^1 = d_{34}^1 = 2$ and 
$d^2_{12} = d^2_{34} = \sqrt{2}$, respectively).  
Despite this, when considering the entire dataset, 
it is not clear that we should believe 
there is any intrinsic association between items 3 and 4 
aside from an overall pattern in buyer behavior.  
%[I think this needs to be tightened up some, to make more convincing.
% The point, which is common, is that there is a meaningful distinction between
% sample and population.
To see this, note that buyers 1-5 bought most available items, 
while buyers 8-12 bought very few items,
and buyers 6 and 7 bought an intermediate number of items.  
The association between items 3 and 4 reflects this pattern in buyers.
%rather than a true underlying association between these items.  
%Items 1 and 2, on the other hand, show similar buying patterns that can {\it not} be explained by buyer differences.  
%%%% [I think this is a false sentence and so am removing it. The fact that only low volume 
%%%% consumers buy these two items in fact means the pattern is potentially due to buyer difference!]
However, buyers who do not purchase many items overall 
still tend to purchase items 1 and 2 together. This is an 
indicator of a true underlying association between these features 
that is interesting in market basket data.



Figure~\ref{fig: toy coh} illustrates the difference 
between correlation and latent association.
Figure~\ref{fig: toy coh}(a) depicts the sample correlation matrix of the toy dataset, 
for which the submatrices associated with item sets
\{1, 2\}  and \{3, 4\} have the same values.  
Figure \ref{fig: toy coh}(b) depicts the latent association matrix
of the toy dataset. It is calculated by the methods outlined in this paper.  
In Figure \ref{fig: toy coh}(b), the item set \{1, 2\} remains associated, 
but other item associations are attenuated, since they
are not distinguishable from the overall pattern among buyers.
For market basket data, the item set \{1, 2\} is an interesting
association mining result, and is the only set of items that the LAMB method declares associated.
The LAMB method correctly regards associations among other possible item sets as noise.
These results are in contrast to conventional methods.
This is discussed further in Appendix~\ref{app: toy data results}.
We discuss throughout the paper how the LAMB method simultaneously 
handles heterogeneity among both observations and features 
(buyers and items in this context) 
through a statistical framework and meaningful 
hypothesis tests.
%by estimating associations between features 
%in a statistically meaningful way.


\begin{figure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = .9\textwidth]{./img/toy_cor_plot.pdf}\\
\hspace{1em}
\caption{Sample correlation}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = .9\textwidth]{./img/toy_coh_plot.pdf}\\
\hspace{1em}
\caption{Estimated latent association}
\end{subfigure}

\caption{Item association matrix comparison for toy market basket dataset.
\red{REDO (b) using new LAMB}}
\label{fig: toy coh}
\end{figure}


%%\subsection{Applications}
%%\label{subsec: notation}
%%
%%\red{What am I trying to accomplish 
%%in this section?! It comes off as very defensive.}
%%\blue{Probably should mention earlier
%%that in Section X we consider 
%%LAMB on non binary datasets
%%and that it performs well.}
%%
%%\blue{Try to answer this: What is the point?}
%%
%%\blue{this paragraph can be 
%%moved because not being used for a while.}
%%We will represent a binary-valued dataset with $n$ samples 
%%and $d$ features by a matrix 
%%$\mathbb{X} = [X_{ij}] \in \{0,1\}^{d \times n}$ in 
%%which columns correspond to samples and rows correspond to 
%%features.
%%In particular, $X_{ij}$ is the value of  feature $i$ in sample $j$. 
%%For example, as noted above, in market basket data
%%$X_{ij}$ is equal to one if buyer $j$ purchases item $i$, 
%%and $X_{ij}$ is equal to zero otherwise. 
%%
%%\red{this is not a great paragraph 
%%because what I'm talking about is not really
%%normalization.}
%%\blue{look up how normalization is used as a word 
%%and what it means}
%%\blue{try something like:
%%The LAMB method can be applied to nonbinary
%%datasets blah blah blah.
%%This sort of transformation may be 
%%appropriate for data that has XYZ}
%%\red{this sounds apologetic:}
%%The LAMB method is only appropriate for samples
%%with  binary-valued features,
%%or features that may be transformed
%%to have binary values.
%%%Not all existing association mining methods are
%%%limited to binary-valued observations.
%%Such transformations of features into binary values
%%can be considered as a normalization step for
%%data that are very sparse or have a low 
%%signal-to-noise ratio or both.\footnote{Sometimes 
%%thresholding count or continuous values
%%into binary values is done to simplify its storage. 
%%(CITE 2006 association mining survey)
%%This is no longer much of a constraint with modern computing
%%resources.}
%%\blue{the footnote is apologetic and should
%%be scrapped. probably ok in dissertation.}
%%This is demonstrated in Section~\ref{sec: real datasets},
%%where two sparse, count-valued datasets 
%%are thresholded into binary-valued datasets.
%%%%These two datasets analyzed by a few methods discussed throughout
%%%%this paper. 
%%
%%Market basket data is not the 
%%only possible application of the LAMB method.
%%Other datasets where the LAMB method's
%%key ideas are advantageous for detecting
%%associated features include 
%%text, gene expression, and network data.
%%%%In these types of data, sample heterogeneity
%%%%is typically present. Accounting for 
%%%%sample heterogeneity and 
%%In these datasets there may be heterogeneity 
%%among the samples and a meaningful notion 
%%of an intrinsic association between features.
%%\red{what does the last part of this sentence mean?!}
%%These two points are discussed
%%in more detail in Section~\ref{sec: real datasets}.
%%

%%Throughout we use language borrowed from Object Oriented Data Analysis
%%to describe samples and variables in a consistent framework.
%%Specifically, data objects will be represented by columns in a data matrix
%%and features will be represented by rows in the same data matrix.
%%Data objects are typically called individual samples from one random sample 
%%and features are typically called variables for the same random sample.

%%%%\subsection{Overview of the LAMB method}
%%%%\label{subsec: lamb overview}
%%%%
%%%%The LAMB method proposed in this paper is based on a simple 
%%%%latent variable model for the binary-valued observations. %(columns) in the data matrix
%%%%%$\mathbb{X} = [x_{ij}]\in\{0,1\}^{d\times n}$.
%%%%Under this generative model
%%%%each observation $\bm{x}_{\cdot j} \in \{0,1\}^d$ is obtained by
%%%%comparing the components of a continuous random vector $\bm{V}_j \in \reals^d$
%%%%to those of an independent random vector of thresholds $\bm{\theta}_j \in (0,1)^d$ 
%%%%via quantile functions.   
%%%%This threshold model is described in Section~\ref{sec:model}.
%%%%%The quantile functions used in the comparison 
%%%%%derive from the marginal CDFs $F_i$ 
%%%%%of the random vectors $C_j$.
%%%%Note that the random vectors $\bm{V}_j$ 
%%%%are \emph{not} assumed to be Gaussian, and the components
%%%%may exhibit complex dependence structure. 
%%%%%The threshold model leads naturally to an association measure between variables based on their latent
%%%%%correlation, defined as the expected correlation of the variables over the joint distribution of $\bm{C}$ and 
%%%%%$\bm{\theta}$. 
%%%%This threshold model leads naturally to an association statistic
%%%%between features that we call latent association;
%%%%the statistic is based on conditional correlation.
%%%%Latent association is explicitly defined in Section \ref{subsec: latent coh}.
%%%%%We extend this pairwise statistic to a statistic 
%%%%%of association between one feature and a set of features
%%%%%by using additivity.
%%%%
%%%%A central limit theorem for latent association
%%%%between a single feature and a set of features,
%%%%with fixed dimension $d$ and growing sample size $n$,
%%%%is established in Section \ref{sec: CLT}.  
%%%%%With estimates of the random thresholds 
%%%%%$\hat{\bm{\theta}}_{\cdot 1}, \ldots, \hat{\bm{\theta}}_{\cdot n}$ in hand, 
%%%%This central limit theorem yields empirical 
%%%%p-values for hypothesis tests of latent association.
%%%%To identify sets of features that have positive latent association,
%%%%we employ an iterative hypothesis testing based search procedure
%%%%using these empirical p-values. %adapted from \citet{ESSC} $\epsilon > 0$.  
%%%%The iterative hypothesis testing algorithm used in the LAMB method is computationally efficient  
%%%%and parallelizable, so it can work on datasets of large size.
%%%%Also, the statistical model used in the LAMB method is able to address data that may 
%%%%yield misleading results in conventional association mining analyses.
%%%%Examples of such misleading results from conventional methods 
%%%%are presented above in this introduction on a toy dataset, 
%%%%and also in Section \ref{sec:model}.
%%%%
%%%%The iterative testing procedure
%%%%used in the LAMB method does not 
%%%%control for False Discovery Rate (FDR) (CITE B-H), 
%%%%but it does incorporate FDR-control per iteration. 
%%%%Such a constraint is important
%%%%due to the multiple comparisons being made 
%%%%in datasets of large size. 
%%%%Conventional methods do not use FDR-control,
%%%%and this is an important part of recent work in association mining.
%%%%(CITE  Pattern Discovery paper, FDR in Association Mining paper, and 2019 robust paper)
%%%%False discoveries from noisy datasets are 
%%%%an important problem that LDA, NMF, and other clustering methods have when applied
%%%%to association mining related datasets.
%%%%(CITE papers!)
%%%%This typically arises as a result 
%%%%of clustering all the data instead
%%%%of only a principled subset of the data.
%%%%We see such false discoveries 
%%%%from these methods in applications to simulated and real datasets, 
%%%%which is discussed 
%%%%in Sections~\ref{sec: sims}, \ref{sec: text}, and \ref{sec: lastfm}.
%%%%
%%%%In order to estimate latent associations between features, 
%%%%we first estimate the unobserved thresholds
%%%%$\bm{\theta}_j$.
%%%%To this end, we assume that the thresholds are generated by a truncated Poisson
%%%%factorization model. This model is discussed in Section~\ref{subsec: theta model}
%%%%and it depends on two parameters that we estimate from the dataset. 
%%%%One parameter is a fixed $d$-vector $\bm{\alpha}$ of rates for each feature. 
%%%%The other parameter is a random $n$-vector $\bm{\tau}$ of rates for each observation;
%%%%the components $\tau_1,\ldots, \tau_n$ are realized values 
%%%%from a random sample of $n$ univariate variables.
%%%%Estimating $\mathbf{\Theta} = [\bm{\theta}_1, \ldots, \bm{\theta}_n] 
%%%%\in (0,1)^{d\times n}$
%%%%is then reduced to estimating the $d + n$ values 
%%%%$(\alpha_1, \ldots, \alpha_i, \ldots, \alpha_d, \tau_1, \ldots, \tau_j, \ldots, \tau_n)$, 
%%%%rather than the $n\cdot d$ values $(\theta_{11}, \ldots,\theta_{ij}, \ldots, \theta_{dn})$.
%%%%In Section~\ref{subsec: parameter consistency}
%%%%we demonstrate the asymptotic consistency for the estimates
%%%%of the parameters $(\alpha_1, \ldots, \alpha_d, \tau_1, \ldots, \tau_n)$.
%%%%
%%%%We wish to use as few distributional assumptions as possible
%%%%for the latent variables to make this method more general. 
%%%%The model for the thresholds above
%%%%is both simple and flexible.
%%%%But we make no such model assumption for 
%%%%the latent random vectors $\bm{V}_j$.
%%%%One downside is this prevents us from explicitly writing out the joint likelihood
%%%%and using Variational Inference (CITE relevant papers)
%%%%or related approximation methods.
%%%%Instead we use an approximation of the joint likelihood
%%%%in the form of a product of marginal likelihoods \blue{(pseudo-likelihood?)}.
%%%%Then an optimization procedure for estimating 
%%%%$(\alpha_1,\ldots, \alpha_d, \tau_1, \ldots, \tau_n)$ 
%%%%from the dataset is applied to this approximated joint likelihood. 
%%%%Details of this implementation are explained in Section~\ref{sec:tildes}.
%%%%%%\red{Say more about TPFM here?}
%%%%
%%%%



\subsection{Organization}
\label{subsec: organization}

The remainder of the paper is organized as follows.
Related work is discussed in Section~\ref{sec: related work}.
The threshold model and latent association components in
the LAMB method are formalized in Section~\ref{sec: model}.
In Section~\ref{sec: search procedure} we outline the
iterative hypothesis testing search procedure
used in the LAMB method.
%including a high-level discussion of the Central Limit Theorem
%that is discussed in detail in Section~\ref{sec: CLT}.
Results from the LAMB method and
other conventional methods applied to real datasets are analyzed
in Section~\ref{sec: applications}.
A simulation study is shown in Section~\ref{sec: sim study}
to see how the LAMB method performs under controlled conditions.
Sections~\ref{sec: CLT} and \ref{sec:params} present 
supporting theoretical results. 
Section~\ref{sec: CLT} goes through the central limit
theorem that is used in the LAMB method's search
procedure. Section~\ref{sec:params} goes through
both the theory and implementation for
estimating the random thresholds 
in the LAMB method's threshold model.




==> tex/model.tex <==

In this section we describe and explore the basic properties of the model framework and the latent association statistic 
used by the LAMB method. 
%In Section~\ref{subsec: threshold model}
%we formulate the model framework for the LAMB method,
%called the threshold model. Then 
%in Section~\ref{subsec: latent coh} we define
%an alternative association statistic, called
%latent association, and describe
%some of its properties. Finally,
%in Section~\ref{subsec: thresh mod intuition}
%we give some intuition for the threshold
%model.


\subsection{Threshold Model}
\label{subsec: threshold model}

The LAMB method is based on a simple threshold model in which
the observed binary-valued vector indicates whether or not
the components of a latent continuous vector lie above or below the corresponding components of a threshold vector. 
We assume that the latent and threshold vectors are random and independent of one another, though the components
of each may be dependent. 
%%However, we do not assume
%%the random thresholds are jointly independent.
%%We are interested in the joint association
%%of the latent continuous vector,
%%so we do not assume that the coordinates
%%of this vector are jointly independent.
The formal definition of the model follows.



\begin{definition}[\textbf{Threshold Model}]
\label{def:mod}
Let $\bm{V}  = (V_1, \ldots, V_d)^T \in \mathbb{R}^d$ be a $d$-dimensional continuous random vector, 
with distribution $\mu$. %such that each component $U_j$ is uniformly distributed.
Let $\bm{\theta} = (\theta_1, \ldots, \theta_d)^T \in (0,1)^d$ be a $d$-dimensional random 
vector, with distribution $\nu$, that is independent of $\bm{V}$.
The random vector $\bm{\theta}$ has a specified structure.
Fix $\bm{\alpha} = (\alpha_1, \ldots, \alpha_d) \in (0,\infty)^d$.  
For each feature $i \in [d]$, let
\begin{align}
	\label{eq:theta}
	\theta_i 
		&:=  1 - \exp(- \alpha_i \tau) \, ,
\end{align}
where $\tau$ is a positive-valued univariate 
random variable with distribution $\pi$.

Under the threshold model, the random vector
$\bm{X} = (X_1, \ldots, X_d)^T \in \{0,1\}^d$ is defined coordinate-wise by
\begin{align}
	\label{eq:thresh}
	X_i 
		&:= \mathbbm{1}\left( V_i \leq F_i^{-1}(\theta_i) \right),
			\quad \textnormal{for } i \in [d] := \{1, \ldots, d\},
\end{align}
where $F_i$ denotes the marginal CDF of random variable $V_i$.
We denote the threshold model in shorthand as
$\bm{X} = \mathbbm{1}\left[ \bm{V} \leq \bm{F}^{-1}( \bm{\theta}) \right]$.
\end{definition}

The role of the random threshold $\bm{\theta}$
in our generative model
is to capture sample heterogeneity.
We impose a structure  on $\bm{\theta}$
that is similar to the 
Poisson factorization approach of \citet{blei}. 
%%The Poisson factorization models expected counts from random sample and variable parameters.
Throughout this paper we refer to the structure
for $\bm{\theta}$ as a truncated Poisson factorization model (TPFM).
Identifiability for the TPFM is discussed in Proposition~\ref{prop: identifiable}.

The form for $\bm{\theta}$ in Definition~\ref{def:mod}
can be thought as arising from a latent ``preference'' vector 
$\bm{Y}$ such that $Y_i | \bm{\alpha}, \tau \sim \textnormal{Poisson}(\alpha_i\tau)$. 
Then the threshold model is equivalent to
\begin{align*}
	\theta_i = \mathbb{P}\left( Y_i > 0 | \bm{\alpha}, \tau\right), 
\end{align*}
for each $i\in[d]$.\footnote{In
copula literature this functional form is called a survival function.}
The parameter  $\tau$ captures  a notion of resource or budget
for the sample, 
while the parameter $\alpha_i$ captures an intrinsic popularity or utility  of feature $i$.
%This assumption for the random thresholds helps us model 
%heterogeneity in observations, i.e.,
%drop the assumption of identically distributed observations.
In particular, we assume that the %association structure and 
randomness of $\bm{\theta}$ derives from a shared univariate random variable $\tau$.  
%%Therefore, in a random sample of thresholds $\bm{\theta}_{\cdot 1},
%%\ldots, \bm{\theta}_{\cdot n}$ the association structure
%%derives from the random sample $\tau_1, \ldots, \tau_n$.
Differences between the marginal distributions of $\theta_1, \ldots, \theta_d$ 
are entirely captured by the fixed parameters 
$\bm{\alpha} = (\alpha_1, \ldots, \alpha_d)$.\footnote{In copula literature
this functional form is called a comonotone copula.}
%In Section~\ref{sec:params} we discuss
%the procedure for estimating these 
%random thresholds.
%If $\tau \sim \textnormal{Gamma}(\zeta, \beta)$, as in Proposition~\ref{prop:prior}, 
%then $Y_i$ is a  Poisson-Gamma random variable for each $i\in [d]$.
%The Poisson-Gamma distributions is common
%in modeling over-dispersed counts.
%%In particular, this model of $\bm{\theta}$ 
%%captures heterogeneity among samples through
%%$\tau$ and heterogeneity among features through $\bm{\alpha}$.


For notational convenience we use quantiles in the threshold model.
This model can also be formulated using copulas. (CITE copula text)
Since $F_i$ is assumed to be a continuous CDF
for each $i\in[d]$, the Probability Integral Transform
implies that $F_1(V_1), \ldots, F_d(V_d)$
are potentially dependent Uniform$(0, 1)$ random variables.
The joint distribution $C$ of $\left(F_1(V_1), \ldots, F_d(V_d)\right)^T$
is called the copula for the joint distribution $F$ of $(V_1, \ldots, V_d)^T$.
In this case the copula $C$ is unique
by Sklar's theorem. (CITE sklar)

Note that we impose no structure on the 
latent continuous vector $\bm{V}$
with joint distribution $F$.
In the LAMB method
there is no inference about the joint
distribution $F$ or marginals $F_1, \ldots, F_d$.
A consequence of not imposing
any structure on $\bm{V}$ is that the threshold model
is not identifiable. Below we give a simple example
of why the threshold model is not identifiable.
The implementation procedure discussed in 
Section~\ref{sec:params} illustrates how
we deal with this in practice.

\begin{example}
\label{ex: threshold model monotone invariance}
Consider a continuous function 
$\gamma\colon \mathbb{R}^d \to \mathbb{R}^d$
with coordinate functions $\gamma_i\colon \mathbb{R} \to \mathbb{R}$
such that, for $i\in [d]$, $x< y$ if and only if $\gamma_i(x) < \gamma_i(y)$.
Denote the joint distribution of  
$\gamma(\bm{V}) = \left(\gamma_1(V_1), \ldots, \gamma_d(V_d)\right)^T$
by $\tilde{F}$ and the marginal distributions of 
$\gamma_i(V_i)$ by $\tilde{F}_i$, for each $i\in [d]$.
A well known result in copula literature is that
copulas are invariant under monotone transformations
of the random variables such as $\gamma(\bm{V})$.
(CITE!) This implies that
the unique copula $C$ for the joint distribution $F$ 
is also the unique copula for 
the joint distribution $\tilde{F}$.
In particular,
\begin{align*}
	\tilde{F}\left(\tilde{F}_1^{-1}(u_1), \ldots, \tilde{F}_d^{-1}(u_d)\right)
		&= C(u_1, \ldots, u_d)
			= F\left(F_1^{-1}(u_1), \ldots, F_d^{-1}(u_d)\right),
\end{align*}
for all $u_i\in (0, 1)$ and $i\in [d]$.
This means that the joint
association structure of $\bm{V}$ captured
by the copula $C$ is invariant
under $\gamma$.
Furthermore, $\tilde{F}_i = F_i\circ \gamma_i^{-1}$ pointwise,
and so $\tilde{F}_i^{-1} = \gamma_i\circ F_i^{-1}$ pointwise.
Finally, note that the threshold model is also invariant
under the transformation $\gamma$:
\begin{align*}
	\mathbbm{1}\left(\gamma_i(V_i) \leq \tilde{F}_i^{-1}(\theta_i)\right)
		&= \mathbbm{1}\left(V_i \leq F_i^{-1}(\theta_i)\right),
			\quad\textnormal{for each}\quad i\in[d].
\end{align*}
This implies that the threshold model
of Definition~\ref{def:mod} is not identifiable.
\end{example}

The threshold model is possibly
invariant to more general transformations
than the function $\gamma$ in the example above.
However, one consequence of %the threshold model 
%being invariant under functions 
%such as $\gamma$ in 
the example above is that the
threshold model effectively
ignores marginal properties such as
location and scale of the
latent continuous vectors. 
%scale invariance is built in to the threshold model. 
This scale invariance allows the LAMB method to 
focus on detecting the joint association structure. 
%\red{Yes or No? : We implicitly assume that $F$
%is a multivariate normal joint distribution
%with unknown mean and unknown variance.}





%\subsection{Model for Random Thresholds}
%\label{subsec: theta model}


%%As noted above, the dependence of $\bm{\theta}$
%%is treated as a nuisance parameter.


%%\blue{
%%Each feature's fixed rate parameter captures intrinsic popularity or usage,
%%while each random parameter captures resource or budget constraints per observation.
%%This assumption for the random thresholds helps us model 
%%heterogeneity in observations, e.g., model differences between high-, intermediate-, 
%%and low-volume buyers independently of intrinsic differences among items.
%%}

%\begin{definition}[\textbf{Threshold Parameter Model}]
%\label{def: threshold model}
%
%\end{definition}







\subsection{Latent Association}
\label{subsec: latent coh}


Suppose that $\bm{X} = \mathbbm{1}\left[ \bm{V} \leq \bm{F}^{-1}(\bm{\theta}) \right]$ 
is generated from the threshold model of Definition~\ref{def:mod}.
Association among $X_1,\ldots,X_d$ arises from two latent sources: association among
the components of the continuous vector $\bm{V}$, and association among the components of 
the threshold vector $\bm{\theta}$.  
We are only interested in the joint
association of $\bm{V}$ and do not
wish to model or estimate $\bm{V}$.
The association among the components of $\bm{X}$ 
arising from thresholds $\bm{\theta}$ is regarded as a nuisance parameter.
%In Section~\ref{subsec: theta model} we describe the 
%model for $\bm{\theta}$ before describing latent association.
We now define the latent association statistic.


\begin{definition}[\textbf{Latent Association}]
\label{def:lat_cor}
Let the binary vector $\bm{X} = \mathbbm{1}\left[ \bm{V} \leq \bm{F}^{-1}( \bm{\theta}) \right]$
be defined as in the threshold model of Definition~\ref{def:mod}.
The latent association $\psi(i, k)$ between $X_i$ and $X_k$ is defined by
\begin{align}
\label{eq:lat_cor}
\psi(i, k)
	&:= \Ex \left( \frac{\left( X_i - \theta_i \right) \left( X_k - \theta_k \right) }{ \sqrt{ \theta_i (1-\theta_i) \, \theta_k (1-\theta_k) } } \right)  .
\end{align}
Here, and in what follows, all expectations are taken with respect to the joint distribution of $(\bm{X}, \bm{\theta})$, 
inherited from the %product 
distribution %$\mu \times \nu$ 
for $(\bm{V},\bm{\theta})$.
\end{definition}

Latent association serves as an appropriate surrogate 
for the association between the features in $\bm{V}$ 
using the observed data $\bm{X}$.
Note that, conditional on $\bm{\theta}$, 
the components $X_1, \ldots, X_d$ of $\bm{X}$ are potentially dependent
Bernoulli random variables with $\mathbb{E}(X_i | \bm{\theta}) = \theta_i$
for each $i\in [d]$.  
It is easy to see that 
\begin{align*}
	\psi(i, k) = \Ex [ \rho(X_i,X_k \given \bm{\theta}) ],
\end{align*}
where $\rho(X_i,X_k \given \bm{\theta})$ denotes the
conditional correlation of $X_i$ and $X_k$ given $\bm{\theta}$.
%which arises from dependence between the latent 
%variables $V_i$ and $V_k$ with fixed thresholds $\theta_i$ and $\theta_k$.   
In particular, $\psi(i, k) = 0$ if $V_i$ and $V_k$ are independent, 
regardless of the distribution of $\bm{\theta}$.
The latent association $\psi(i, k)$ is not a formal parameter of the threshold model of
Definition~\ref{def:mod}, because it does not determine the joint distribution of $\bm{V}$ and $\bm{\theta}$.



In Section~\ref{sec: intro} we provided an 
illustration of the importance of measuring latent association 
rather than standard correlation when sample
heterogeneity is present in a dataset. %on a toy market basket dataset.  
Now we give an explicit example in which $\bm{X}$ has standard correlation
induced by $\bm{\theta}$, despite independence in $\bm{V}$.

\begin{example}
\label{ex1}
	Let $\bm{V} \sim \mathcal{N}_d(\bm{0}, \mathbf{I}_d)$, where 
	$\mathbf{I}_d$ is the $d \times d$ identity matrix.  Let $\theta_1 = \ldots = \theta_d$
	such that, for some $\epsilon \in\left(0, \frac{1}{2}\right)$, we have
	\begin{align}
		\theta_1	\, = \, \begin{cases}
      		\epsilon & \text{ with probability } \, 1/2, \\
    		1 - \epsilon & \text{ with probability } \, 1/2.
  	 \end{cases}
	\end{align}
	Let $\bm{X}$ be as in Definition \ref{def:mod}, 
	i.e., $\bm{X} = \mathbbm{1}\left[ \bm{V} \leq \bm{\Phi}^{- 1}_{\mathbf{I}_d}(\bm{\theta})\right]$
	in our notation, where $\Phi_{\mathbf{I}_d}$ denotes
	the joint CDF for a $\mathcal{N}_d(\bm{0}, \mathbf{I}_d)$ random vector.  
	Then, for any $i \neq k$, $V_i$ is independent of $V_k$ and so
	\begin{align*}
		\mathbb{E}(X_i X_k) - \mathbb{E}(X_i) \mathbb{E}(X_k)
			&= %\left( \frac{\epsilon^2}{2} + \frac{ (1-\epsilon)^2 }{2} \right) - \frac{1}{4} =
				 \frac{1}{4} - \epsilon (1 - \epsilon) \, .
	\end{align*}
	Therefore, the correlation $\rho(X_i, X_k)$
	between $X_i$ and $X_k$ is positive.
	It is easy to see that as $\epsilon$ approaches 0, 
	the correlation between $X_i$ and $X_k$ gets arbitrarily close to $1$.
	
	Intuitively, this dependence arises from the individual variables 
	$V_i$ being simultaneously thresholded at either very
	large or very small values of $\theta_i$, so that $X_i = X_k$ with 
	high probability for any distinct pair $(i,k)$.  
	Standard correlation correctly indicates
	that there is association between the features in $\bm{X}$.  
	However, this association derives from joint association in
	$\bm{\theta}$, instead of joint association in $\bm{V}$.
	Whenever the joint association in $\bm{V}$ is of primary interest, 
	and $\bm{\theta}$ is ancillary to the analysis,
	standard correlation is misleading.
	By contrast, the latent association $\psi(i, k)$ is equal to 0 for any $(i,k)$,
	which accurately reflects the underlying lack of joint association structure in $\bm{V}$.
\end{example}

%\red{Perhaps better to move this to the related work section, and expand the discussion a bit.}

\begin{remark}
The above example is not exceptional.
% \blue{[Insert law of total covariance calculation here.]}
The Law of Total Covariance yields
\begin{align}
	\text{Cov}(X_i, X_k)
%		&= \mathbb{E}\left(\text{Cov}[X_i, X_k| \bm{\theta}]\right)
%			+ \text{Cov}\left(\mathbb{E}[X_i | \bm{\theta}], \mathbb{E}[X_k | \bm{\theta}]\right)\\
		&= \mathbb{E}\left(\text{Cov}[X_i, X_k| \bm{\theta}]\right)
			+ \text{Cov}\left(\theta_i, \theta_k\right).
		\label{eq: law of total covariance}
\end{align}
In association mining, we are not interested in 
association between variables $X_i$
and $X_k$ arising 
from $\text{Cov}\left(\theta_i, \theta_k\right)$. 
The  $\text{Cov}\left(\theta_i, \theta_k\right)$ term
arises entirely from association between sample ``preferences''
$\theta_i$ and $\theta_k$, 
rather than intrinsic association between features.
Under the threshold model, intrinsic association between features %$i$ and $k$ 
is captured by $\textnormal{Cov}(V_i, V_k)$.
The LAMB method estimates association 
between the features of the latent vector $\bm{V}$
from observation of $\bm{X}$ using the 
$\mathbb{E}\left(\text{Cov}[X_i, X_k| \bm{\theta}]\right)$ 
term in Equation~\eqref{eq: law of total covariance}.
\end{remark}

%%As justified by the additive partition in~\eqref{eq: law of total covariance}
%%from the Law of Total Covariance,
%%$\psi(i, k)$ captures dependence between the latent variables $V_i$ and $V_k$.
%%Simultaneously, $\psi(i, k)$ mitigates the effects of the thresholds 
%%$\bm{\theta}$ on measuring this dependence using the observations $X_i$ and $X_k$.



%%%\red{Maybe the following should be moved up?}
%%%We also remark here that one common measure of association between binary variables $X_i$ and $X_k$ is the odds ratio
%%%\[
%%%{\prob{ X_i = 1,  \, X_k =  1 } \prob{ X_i = 0,  \, X_k =  0 } \over \prob{ X_i = 0,  \, X_k =  1 } \prob{ X_i = 1,  \, X_k =  0 }}.
%%%\] 
%%%However, we decide to focus on latent association, 
%%%since the Threshold Model of Definition~\ref{def:mod} 
%%%is reasonable for many practical problems.
%%%Furthermore, latent association incorporates the 
%%%generative model for handling heterogeneity,
%%%and is more related to our goal of recovering the dependence structure in $\bm{V}$ 
%%%while mitigating the effects from the dependence structure in $\bm{\theta}$.
%%%



Latent association shares some of the basic properties of standard correlation.
For example, $|\psi(i,k)| \leq 1$ (see Lemma \ref{lem:uv}) and
$\psi(i,k) \neq 0$ implies dependence between $V_i$ and $V_k$.
Although the latent association of two features in $\bm{X}$ is not necessarily equal to the correlation
of the same two features in the latent vector $\bm{V}$, there is a monotonic relationship when $\bm{V}$ is 
multivariate normal.

\begin{prop}
\label{prop:rho}
Let $\bm{X} = \mathbbm{1}\left[ \bm{V} \leq \bm{F}^{-1}(\bm{\theta}) \right]$  as in Definition~\ref{def:mod}, where
%$\bm{C} \sim \mathcal{N}_d({\bf 0}, \Sigma)$ with $\Sigma_{jj} = \sigma^2$ for all $j$.
$\bm{V} \sim \mathcal{N}_d({\bm{0}}, \mathbf{\Sigma})$ such that $\Sigma_{ii} = 1$, for each $i\in[d]$. 
Then %, for any fixed random vector $\bm{\theta}$, 
$\psi(i,k)$ is a monotone 
nondecreasing function of $\rho(V_i, V_k) = \Sigma_{ik}$.
%\beq
%\label{eq:psipos}
%%\mbox{sgn}(\psi(j,k)) = \mbox{sgn}(\Sigma_{jk}) \, 
%\eeq
%i.e., the sign of the latent coherence between $X_i$ and $X_i$ is equal to the sign of the
%correlation between $V_i$ and $V_j$.
\end{prop}

The proof of Proposition~\ref{prop:rho}
is in Appendix~\ref{app:theory},
and the key step in the proof is using Slepian's Lemma.
We note that the LAMB method described below 
does not explicitly rely on normality assumptions for $\bm{V}$.
However, the above proposition states that whenever $\bm{V}$ is 
multivariate normal, 
latent association is guaranteed to be
a monotone nondecreasing function 
of the correlation between components 
of $\bm{V}$.\footnote{This is useful if one can shown
there exists a function $\gamma\colon \mathbb{R}^d\to\mathbb{R}^d$, such as in 
Example~\ref{ex: threshold model monotone invariance},
that can a map general latent continuous vector
$\bm{V}$ with a given CDF $F$
to a multivariate normal random vector $\gamma(\bm{V})$.}
Note that this matches intuition for the generative model: if the correlation between
$V_i$ and $V_k$ is increasing, then the latent association $\psi(i,k)$
is monotonically nondecreasing.\footnote{In our
simulation study we see that the sample estimate of $\psi(i, k)$ increases
as the true underlying correlation increases, within some small error.}

Latent association can be expressed as a functional 
of the joint and marginal CDFs for $\bm{V}$. 
In particular, this clearly illustrates why
$\psi(i,k) = 0$ whenever $V_i\indep V_k$.
The functional form of latent 
association also shows that 
if $C_1$ and $C_2$ are two copulas 
such that $C_1 \prec C_2$, then
the corresponding latent associations
$\psi_1(i, k)$ and $\psi_2(i, k)$
satisfy $\psi_1(i, k) \leq \psi_2(i, k)$.
See Propositions~\ref{prop: dist functional}
and \ref{prop: concordance monotonicity} in Appendix~\ref{app:theory}
for details. \red{Add a sentence about why this 
is nice.}


\subsection{Intuition for the Threshold Model}
\label{subsec: thresh mod intuition}


Following the discussion in Section~\ref{sec: intro},
we provide some intuition behind this generative model
for market basket data. %and text data.
In this context the vector $\bm{F^{-1}(\theta)} := (F_1^{-1}(\theta_1),
\ldots, F_d^{-1}(\theta_d))^T$ represents the 
preferences of an individual buyer. %purchasing items $1, \ldots, d$.
%In particular, 
In particular, the variable $F_i^{-1}(\theta_i)$ represents the 
preference of an individual buyer to purchase item $i\in [d]$:
\begin{align*}
	F_i^{-1}(\theta_i)
		&= F_i^{-1}\left(\mathbb{P}[\textnormal{ buyer purchases item $i$ } | \bm{\alpha}, \tau] \right).
\end{align*}
We interpret $\tau$ as the buying propensity 
or budget resource of an individual buyer randomly selected from the population, 
and $\alpha_i$ as a measure of overall popularity or utility of item $i\in [d]$.
The truncated Poisson factorization model
of the random threshold vector $\bm{\theta}$
captures heterogeneity among the population's item
preferences, and heterogeneity among different buyers
propensities or resources.
%See Section~\ref{subsec: theta model} for details
%about the truncated Poisson factorization model.
%\red{probably need to move theta model up here}

Scale invariance
of both the threshold model
and the copula representing the joint association structure 
was discussed in Section~\ref{subsec: threshold model}.
This scale invariance simplifies the interpretation of $\bm{V}$.
The continuous random vector $\bm{V}$ represents the joint 
``luxury''  of purchasing the $d$ items
for an individual buyer. 
Larger values of $V_i$ represent
items that have a larger personal cost
to an individual buyer. 
Items that simultaneously have lower
personal costs to an individual buyer
are more likely to be purchased together,
and these items are likely associated in 
the context of market basket data.

%%In context of text data, terms have different ``limits'' of meaning or use. 
%%Certain terms are more convenient and others are more specialized. 
%%Larger values of $V_i$ represent a more limited or specialized term
%%and smaller values of $V_i$ represent a less limited or specialized term.
%%Terms may exhibit complex dependence structures for different reasons, 
%%e.g., topical or grammatical. 
%%While in this context the variable $F_i^{-1}(\theta_i)$ represents the 
%%preference of using term $i$ in the text document.
%%
%%
%%For text data we interpret $\tau$ as capturing the verbosity of the document source or author
%%and $\alpha_i$ as capturing the semantic utility of a term.







==> tex/rel_work.tex <==
The LAMB method addresses the problem of
identifying sets of features with positive associations
in a sample of binary-valued observations.  
Existing work addressing this problem
is predominantly called
Frequent (or Interesting) Pattern Mining
in data mining literature. 
Pattern mining methods 
have roots in the work of \citet{apriori}, 
which introduced the \texttt{apriori} algorithm.
Subsequent methods made algorithmic solutions 
and computational improvements to the \texttt{apriori} algorithm.  
Some notable examples include  \texttt{eclat} \citep{eclat},
\texttt{MAFIA} \citep{mafia}, 
\texttt{COBBLER} \citep{cobbler}, 
\texttt{fp-close} \citet{fpclose},
and  \texttt{CHARM} \citep{charm}.  
The work in (CITE Brin et al.) discusses 
the importance of searching for dependence,
as opposed to just frequency, 
in a pattern mining method.
A summary of early and recent work in 
pattern mining can be found in \citet{zaki}, \citet{survey2013}, \cite{zaki1999parallel},
(CITE FPM AGGAREAL TEXT), (CITE SURVEY PAPERS and Zaki), and the references therein.  





In general, the pattern mining approaches referenced above are non-stochastic.
There are some stochastic or model-based pattern mining methods.  
For example, \citet{prob_data} is one such stochastic method.
More complex, model-based approaches can be found in 
\citet{Aggarwal_uncertain} and \citet{tong_chen_cheng_yu_2012}.


Computationally, pattern mining methods 
can handle datasets that have a large number of observations, 
but only a moderate number of features (e.g., $10^2$ or fewer).  
More recent work in pattern mining attempts to
address the challenge of high-dimensional datasets.
For important examples, 
see \citet{liu_colossal}, \citet{Sohrabi_colossal}, and \citet{zhu_colossal}.  
Small-data methods are still the norm in pattern mining analyses.

An alternative to pattern mining methods
for addressing this problem is clustering 
and normalization.
Clustering features in a sample of 
binary-valued observations is possible,
we simply specify an appropriate measure 
of distance or dissimilarity. 
Some of these binary measures are provided in 
\citet{binary_survey} and \citet{nobel_2008}. 
\red{This reference is pretty obscure.  It would be good to have
references to core literature, e.g., surveys.-Andrew}
A general framework and discussion of methods for clustering 
binary-valued datasets can
be found in \citet{Li_unified} and \citet{Li_clustering}; a survey of classic approaches is given in \citet{corr_bin_dat}.
Latent space regression models can be partially adapted to unsupervised clustering tasks, as discussed in 
\citet{subspace} and \citet{dunson_2000}.  \red{Worth looking at other work of Dunson.-Andrew}
Related literature for the task of identifying sets of features 
using clustering can be found in \citet{corrclust} 
and the references therein.
\red{(Add other citations?)}  

By applying a normalization method,
usually per observation,
binary-valued data may be transformed into
real-valued data. Such a normalization 
may be combined with an appropriate 
clustering method to cluster features
in a sample of observations.
Commonly used normalization methods
are $L^2$-normalization, $L^1$-normalization, and
Term frequency Inverse document frequency (Tf-Idf) normalization.
(CITE RELAVENT PAPER, see Original LDA intro)
A Tf-Idf analysis is supplied alongside the LAMB results in Section \ref{sec: text}.


The LAMB method assumes that binary-valued 
observations arise from a random thresholding of a 
latent continuous random vector.
Treating binary data as thresholded continuous data is a common practice in regression models,
see for example \citet{latent1}, \citet{latent2}, \citet{latent3}.  In typical regression models it is assumed that
binary observations derive from a much lower dimensional structure and high dimensional noise.
By contrast, our model assumes that the observed binary vector  and 
the unobserved continuous random vector 
have the same dimension $d$, and
concern the same quantities of interest.  
The threshold models employed in regression 
generally account for random noise in the latent variables,
but typically assume a fixed thresholding process.

Other commonly used data mining methods
can also address the problem of 
identifying sets of features with positive associations
in a sample of binary-valued (or count-valued) observations.  
Much like regression models, 
Latent Semantic Analysis (LSA)--sometimes
called Latent Semantic Indexing (LSI)--uses
a latent, low-rank model to lower the underlying dimension of the data.  
See \citet{lsa_classic}, \citet{landauer_2006}, 
(CITE Aggarwal ML), and the references therein for an overview of LSA.  
A similar latent, low-rank method is Nonnegative Matrix Factorization (NMF).
(CITE Aggarwal and Lee and Seung Learning Parts)
(CITE Lee and Seung NMF algorithms)

More modern versions of NMF can be found 
in the review paper (CITE IEEE NMF Review) and references therein.
For details relating to unique decompositions by NMF see (CITE Donoho NMF),
where they consider the geometry of the problem.
We note that there is a version of NMF that focuses on binary matrices,
called Binary Matrix Factorization. (CITE BMF with Applications IEEE)
However, because we consider count-valued datasets in our applications and
NMF performs accurately on the simulated binary datasets,  
we chose to focus on comparing the LAMB method 
to the more general NMF method.
Note that NMF can be viewed as a generative mixture model. Other 
generative mixture models include Bernoulli or Multinomial models.
(CITE RELAVENT PAPERS)

A probabilistic model that addresses 
heterogeneity in both features and observations,
similar to the LAMB method, 
is Latent Dirichlet Allocation (LDA). (CITE Original LDA paper)
The latent variables in LDA are often called topics.
An important feature of LDA, and similarly NMF, is 
that the method allows for mixed-membership of topics within observations 
and features within topics. 
This allows LDA to handle complex association 
structure between features in general. (CITE Steyvers and Griffths Probabilistic Topic Models)
There are a few different ways to describe the generative process of LDA,
and also many extensions of the original LDA method,
but a good description is provided in (CITE Blei Lafferty Topic Models).


We note here that the idea of latent association is related to the idea of 
the tolerance distribution interpretation in classical 
generalized linear models \citep{mccullagh1989generalized}
through the introduction of latent variables.
\red{(Please check and expand this.  More references? -Andrew)}



%(Briefly mention \citet{ESSC} and other papers using iterative testing based search strategy.)
The iterative based hypothesis testing idea 
used in the LAMB method has been used in other work, 
see (CITE RELEVANT PAPERS). 
In LAMB and the other works, 
approximate p-values 
are used with multiple-testing procedures 
to control false discovery rates per iteration.
Such a procedure aims to identify statistically 
significant clusters or communities, 
depending on the context. 
In particular, this procedure identifies background noise 
from the data. 
This is useful when dealing with real data sets.



\blue{Find a place to add this: (see \citep{binary_survey} for a survey of binary distance measures)}

\blue{Find a place for this: Application of some latent variable methods discussed below to biological data 
can be found in (CITE Holmes Microbiome).}


